On methods for correcting for the look-elsewhere effect in searches for new physics

The search for new significant peaks over a energy spectrum often involves a statistical multiple hypothesis testing problem. Separate tests of hypothesis are conducted at different locations producing an ensemble of local p-values, the smallest of which is reported as evidence for the new resonance. Unfortunately, controlling the false detection rate (type I error rate) of such procedures may lead to excessively stringent acceptance criteria. In the recent physics literature, two promising statistical tools have been proposed to overcome these limitations. In 2005, a method to "find needles in haystacks" was introduced by Pilla et al. [1], and a second method was later proposed by Gross and Vitells [2] in the context of the "look elsewhere effect" and trial factors. We show that, for relatively small sample sizes, the former leads to an artificial inflation of statistical power that stems from an increase in the false detection rate, whereas the two methods exhibit similar performance for large sample sizes. We apply the methods to realistic simulations of the Fermi Large Area Telescope data, in particular the search for dark matter annihilation lines. Further, we discuss the counter-intutive scenario where the look-elsewhere corrections are more conservative than much more computationally efficient corrections for multiple hypothesis testing. Finally, we provide general guidelines for navigating the tradeoffs between statistical and computational efficiency when selecting a statistical procedure for signal detection.

==> JINST.cls.1.0.1 <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% JINST.cls 1.0.1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% This file is Copyright JINST 2006:  it can be freely distributed  but
%% NOT modified preserving its name, even in similar forms.
%% 
%% JINST.cls is a LaTeX2e class file used to typeset manuscripts in 
%% Journal of Instrumentation (http://jinst.sissa.it) style. It was 
%% written by P. Dall'Aglio as a modification of the class JHEP3.cls 
%% 
%% JINST.cls is only for internal use of the JINST typesetting office.
%% 
%% For bugs, comments, suggestions email to jinst-eo@jhep.sissa.it
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesClass{JINST} [2006/07/11 v1.0.1 LaTeX document class - P.D.]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\logo{\raisebox{-10.5\p@}{\hb@xt@85\p@{\includegraphics{JINSTlogo}\hfil}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW SWITCHES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if@preprint\@preprinttrue		% DEFAULT IS PREPRINT!
\newif\if@draft   \@draftfalse			% DEFAULT IS NOT DRAFT
\newif\if@hyper   \@hypertrue			% DEFAULT IS HYPER
\newif\if@proc	  \@procfalse			% DEFAULT IS NOT PROC

\newif\if@author\@authorfalse			%
\newif\if@abstract\@abstractfalse		% FOR FRONTMATTER DECLARATIONS
\newif\if@keywords\@keywordsfalse		%
\newif\if@todotoc\@todotocfalse			%
\newif\if@rece\@recefalse			%
\newif\if@revi\@revifalse			%
\newif\if@acce\@accefalse			%
\newif\if@publi\@publifalse			%
\newif\if@Jcopy\@Jcopyfalse			%
\newif\if@conf\@conffalse			%
\newif\if@Jspecialurl\@Jspecialurlfalse
\newif\if@Jcits\@Jcitsfalse
\newif\ifpdf
\ifx\pdfoutput\undefined
\else
  \ifx\pdfoutput\relax
  \else
    \ifcase\pdfoutput
    \else
      \pdftrue
    \fi
  \fi
\fi


\if@compatibility
    \setlength\paperheight {297mm}%		% DEFAULT FOR LATEX209 IS a4
    \setlength\paperwidth  {210mm}%
\else						% CHOSE PAPER:
\DeclareOption{a4paper}
   {\setlength\paperheight {297mm}%
    \setlength\paperwidth  {210mm}}
\DeclareOption{a5paper}{\@OImess{}}		% IGNORED a5
\DeclareOption{b5paper}{\@OImess{}}		% IGNORED b5
\DeclareOption{letterpaper}
   {\setlength\paperheight {11in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{legalpaper}
   {\setlength\paperheight {14in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{executivepaper}
   {\setlength\paperheight {10.5in}%
    \setlength\paperwidth  {7.25in}}
\DeclareOption{landscape}{\@OImess{}}		% IGNORED landscape
\fi

\newcommand\@ptsize{1}                          % DEFAULT SIZE IS 11 PT

\DeclareOption{published}{%
\ifpdf
%\JINST@warnl{Option 'published' incompatible with 
%pdf output, turning to dvi output}\pdffalse\pdfoutput=0
\@preprintfalse
\else
\@preprintfalse%
\fi}
\DeclareOption{nocits}{\if@preprint\@OImess{ is default for preprints}\else
		       \@Jcitsfalse
                       \fi}

\DeclareOption{cits}{%\if@preprint
                     \@Jcitstrue %\else
                     %\@OImess{ is automatic for published papers}\fi
                     }	

\DeclareOption{hyper}{\@hypertrue}	% HYPER IS 11 PT
\DeclareOption{nohyper}{\@hyperfalse}	% PAPER IS ALSO 11 PT (v1.3)
\DeclareOption{paper}{\@hyperfalse}	% PAPER IS ALSO 11 PT
\DeclareOption{11pt}{\renewcommand\@ptsize{1}\ExecuteOptions{@FONT}}
\DeclareOption{12pt}{\renewcommand\@ptsize{2}\ExecuteOptions{@FONT}}
\if@compatibility\else                          % LATEX2.09 HAS NO 10PT 
\DeclareOption{10pt}{\renewcommand\@ptsize{0}\ExecuteOptions{@FONT}}% v1.4
\fi       				% CHOSEN TO FREE MEMORY LATER:
\DeclareOption{@FONT}{\if@preprint              % IF PREPRINT ALLOW ANY,
                        \else			              % IF PUBLISHED: 
			\renewcommand\@ptsize{1}\@NFmess{11pt}% ALWAYS 11PT
                        \fi
			}
                        
\if@compatibility\else
\DeclareOption{oneside}{\@twosidefalse \@mparswitchfalse}\fi
\DeclareOption{twoside}{\if@preprint\if@hyper\@OImess{ in hyper-mode}
				    \else\@twosidetrue\@mparswitchtrue\fi
			\else			% FOR PUBLISHED
			\@OImess{ in published papers}
			\fi}
\DeclareOption{notoc}{\if@preprint		% to disable TOC
			\AtBeginDocument{\@todotocfalse}
			\else
			\@OImess{ in JINST papers}
			\fi}
\DeclareOption{draft}{\setlength\overfullrule{5pt}% EXTENDED DRAFT
	\newcount\hour\newcount\minute
	\hour=\time \divide\hour by60 \minute=\time
	{\multiply\hour by60 \global\advance\minute by-\hour}
	\edef\militarytime{\number\hour:\ifnum\minute<10 0\fi\number\minute}
	\let\old@eqnnum\@eqnnum
	\def\@eqnnum{\old@eqnnum\rlap{\kern\marginparsep
				\if@twocolumn\if@firstcolumn
				  \kern-2\marginparsep\kern-\columnwidth\
				  \llap\bgroup\else\bgroup\fi
				\else
				\if@twoside\ifodd\c@page
				  \kern-2\marginparsep\kern-\textwidth
				  \llap\bgroup\else\bgroup\fi
				\else\bgroup\fi				
				\fi
				\sf\scriptsize\@eqnlabel\egroup}%
				\gdef\@eqnlabel{}}
	\let\@eqnlabel\relax
	\def\math@note#1{\gdef\@eqnlabel{LAB: #1}}
	\def\norm@note#1#2{\special{}% SORRY AGAIN.
			 \ifinner{\ifdim\baselineskip=\z@% IN ARRAY..
					\baselineskip18\p@\fi%%
				\ifhmode%   ATTENTION TO RESTRICTED VMODE!
				\raisebox{.5\baselineskip}[\z@][\z@]{%
					\rlap{\sf\scriptsize #2}}%
				\else\vskip-\baselineskip%
				\raisebox{-.6\baselineskip}[\z@][\z@]{%
						\rlap{\sf\scriptsize #2}}%
				\fi}%
			 \else\marginpar{\raggedright\if@twoside\ifodd\c@page%
					\raggedleft\fi\fi\sf\scriptsize #1#2}%
			 \fi}%
	\AtBeginDocument{\newbox\drft@box\setbox\drft@box=\hbox{%
			\framebox[\textwidth]{\sf\small JINST DRAFT 
			\ttfamily(\cur@opt)\hfill\sf\bfseries\jobname\sf, 
			\today, \militarytime}}}
	\@drafttrue}

\DeclareOption{titlepage}{\@OImess{}}		% IGNORED
\if@compatibility\else
\DeclareOption{notitlepage}{\@OImess{}}		% IGNORED
\fi
\if@compatibility\else
\DeclareOption{onecolumn}{\@OImess{}}		% IGNORED
\fi
\DeclareOption{twocolumn}{\@OImess{}}		% IGNORED
\DeclareOption{leqno}{\@OImess{}}	%\input{leqno.clo}} IGNORED ...
\DeclareOption{fleqn}{\@OImess{}}	%\input{fleqn.clo}} IGNORED ...
\DeclareOption{openbib}{\@OImess{}}		% IGNORED


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MESSAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\JINST@mess[1]{\typeout{Class JINST Message: \protect#1.}}%
\newcommand\JINST@warn[1]{\ClassWarning{JINST}{#1}}
\newcommand\JINST@warnl[1]{\ClassWarningNoLine{JINST}{#1}}
\newcommand\JINST@igno[1]{\JINST@warn{IGNORED \protect#1}}
\newcommand\JINST@ignol[1]{\JINST@warnl{IGNORED \protect#1}}
\newcommand\@OImess[1]{\JINST@ignol{OPTION '\CurrentOption'#1}}
\newcommand\@NFmess[1]{\JINST@mess{Normalsize set to #1}}
\newcommand\@ENVwarn[1]{\JINST@warn{Please use \protect#1 in place 
						of LaTeX environment}}
%%%%%%%%%%%%%%%%%%%%%%%%%% PROCESS OPTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ExecuteOptions{a4paper,oneside,hyper} %WERE ALSO 10pt,onecolumn
\ProcessOptions

%%%%%%%%%%%%%%%%%%%%%%%%%% REQUIRED PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{amssymb}
\RequirePackage[T1]{fontenc}
\RequirePackage{times}
\RequirePackage{mathptmx}
\ifpdf
      \RequirePackage[pdftex]{graphicx}
      \DeclareGraphicsExtensions{.pdf,.jpg,.jpeg}
\else
      \RequirePackage{graphicx}
      \DeclareGraphicsExtensions{.ps,.eps,.pstex}
\fi
%%%%%%%%%%%%%%%%%%%%%%%% TRICKS FOR DOTLESS J %%%%%%%%%%%%%%%%%%%%%%%%%
%\j and \jmath are missing in font Times. So I use the ones from
% Computer Modern. Works acceptably, but in sf
\DeclareSymbolFont{forjmath}{OT1}{cmr}{m}{sl}
\DeclareMathSymbol{\Jmath}{\mathord}{forjmath}{'021}
\def\jmath{\Jmath}
\DeclareFontFamily{OT1}{cmr}{}
\DeclareFontFamily{OT1}{cmss}{}
\def\j{\ifmmode\Jmath\else{\fontencoding{OT1}\fontfamily{cmr}\selectfont\char'021}\fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END DOTLESS J %%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% START CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{size1\@ptsize.clo}
\renewcommand{\baselinestretch}{1.1}\normalsize
\setlength\lineskip{1\p@}
\setlength\parindent{1.2\parindent}	% AT 12pt 1.5em BECOMES 1.8em=tocindent
\setlength\normallineskip{1\p@}
\setlength\parskip{0\p@ \@plus \p@}
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
\widowpenalty 1000
\clubpenalty 1000

\setcounter{topnumber}{4}
\renewcommand\topfraction{1} % default .7
\setcounter{bottomnumber}{1}
\renewcommand\bottomfraction{.6} %.2		% .6 ???***
\setcounter{totalnumber}{5}
\renewcommand\textfraction{0}
\renewcommand\floatpagefraction{1}
\setcounter{dbltopnumber}{3}
\renewcommand\dbltopfraction{.7}
\renewcommand\dblfloatpagefraction{1}

\textwidth  .72\paperwidth	% WIDTH OF TEXT, REMAINS .28% FOR MARGINS
%
\setlength\@tempdima{.76\paperheight}	% HEIGHT OF TEXT WITH FOOTNOTES
\divide\@tempdima\baselineskip		% EXCLUDING HEAD (AND FOOT)
\@tempcnta=\@tempdima			% rounded to integer (#lines-1)
\setlength\textheight{\@tempcnta\baselineskip}
\addtolength\textheight{\topskip}

\voffset -1in
\topmargin   .05\paperheight	% FROM TOP OF PAGE TO TOP OF HEADING (0=1inch)
\headheight  .02\paperheight	% HEIGHT OF HEADING BOX.
\headsep     .03\paperheight	% VERT. SPACE BETWEEN HEAD AND TEXT.
\footskip    .07\paperheight	% FROM END OF TEX TO BASE OF FOOTER. (40pt)

\marginparsep 9\p@		% HOR. SPACE BETWEEN TEXT AND MARGINAL NOTE
\marginparpush 6\p@		% MIN. VERT. SPACE BETWEEN MARGINAL NOTES

\hoffset -1in				% TO ADJUST WITH PAPER:
\if@twoside				% IF TWO-SIDED:
	\oddsidemargin .13\paperwidth	% LEFT MARGIN FOR ODD PAGES (10)
	\evensidemargin .15\paperwidth	% LEFT MARGIN FOR EVEN PAGES (30)
	\marginparwidth .10\paperwidth	% TEXTWIDTH OF MARGINALNOTES
	\reversemarginpar		% BECAUSE OF TITLEPAGE.
\else					% IF ONE-SIDED:
	\oddsidemargin .14\paperwidth	% LEFT MARGIN FOR ODD PAGES (20)
	\evensidemargin .14\paperwidth	% LEFT MARGIN FOR EVEN PAGES (20)
	\marginparwidth .11\paperwidth	% TEXTWIDTH OF MARGINALNOTES
\fi					%
%%%%%%%%%%%%%%%%%%%%%%% HYPER (AND DRAFT) STUFF %%%%%%%%%%%%%%%%%%%%%%%
\ifpdf
      \input pdfcolor.tex
\else
\fi

\bgroup\catcode`\#=12\gdef\hash{#}\egroup	% DEFINED \hash=#.
\def\H@tilde{\string~}
\newcommand{\href}[2]{\rule{0pt}{0pt}\bgroup\let~\H@tilde
		      \if@hyper\ifpdf
				    \def\hash{}%
				    \pdfstartlink attr{/Border [1 1 1] /C [0 0 1]}
                                    user{/Subtype /Link /A << /S /URI /URI (#1) >>}%
					\pdfsetcolor{0 0 0 1}%
				\else
				    \noexpand\special{html:<A href="#1">}%
				\fi
		      \fi
		      \rule{.2ex}{0pt}\rule[-.5ex]{0pt}{2.2ex}{#2}\rule[-.5ex]{0pt}{2.2ex}\rule{.1ex}{0pt}\egroup
		      \if@hyper\ifpdf
				    \Black\pdfendlink
			       \else
				    \special{html:</A>}%
			       \fi
                      \fi
		      }
% \intPlink was added because in pdflatex you need two different commands
% for internal and external links. For latex they are the same.
\newcommand{\intJlink}[2]{\rule{0pt}{0pt}\bgroup\let~\H@tilde
                        \if@hyper\ifpdf
                                       \def\hash{}%
                                       \pdfstartlink attr{/Border [1 1 1] /C [0 0 1]}
                                          goto name{#1}%
                                       \pdfsetcolor{0 0 0 1}%
				  \else
                                       \noexpand\special{html:<A href="#1">}%
				  \fi
			\fi
                        \rule[-.2ex]{0pt}{1.8ex}{#2}\rule[-.2ex]{0pt}{1.8ex}\egroup
                        \if@hyper\ifpdf
                                      \Black\pdfendlink
				 \else
                                      \special{html:</A>}%
                                 \fi
                        \fi
                        }


\newcommand{\name}[1]{{\if@hyper\ifpdf
				    \pdfdest name{#1} fith%
			       \else
				    \noexpand\special% NAME HAS NO TAGGED TEXT HERE.
					{html:<A name="#1">}\special{html:</A>}%
			       \fi
		      \fi}%
		      }
\newcommand{\base}[1]{\if@hyper\ifpdf
                        \relax\JINST@warn{Command base undefined for pdf output}
			%\pdfdest baseurl{#1} fith%
                       \else
                        \bgroup\let~\H@tilde
			\noexpand\special	% BASE HAS NO TAGGED TEXT.
			{html:<base href="#1">}\egroup
                       \fi\fi}
%------------------------------------------------------------------%
% SECTION TAGS and  THEIR REFERENCE IN TOC \d@t will be '.' for sections only
\if@hyper
\renewcommand{\@seccntformat}[1]{\name{sec\csname the#1\endcsname}%
				 \csname the#1\endcsname\d@t\hspace{1ex}}
\renewcommand{\numberline}[1]{\hb@xt@\@tempdima{\intJlink
			      {\hash\hyp@typ#1}{#1}\d@t\hfil}}
\else
\renewcommand{\@seccntformat}[1]{\csname the#1\endcsname\d@t\hspace{1ex}}
\renewcommand{\numberline}[1]{\hb@xt@\@tempdima{#1\d@t\hfil}}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% this is to obtain collapsing citations %%%%%%%%%%%%%%%%%%
\if@Jcits                             % only if 'cits' option is chosen
\newcount\@tempcntc
\def\@citex[#1]#2{%
  \@tempcnta\z@\@tempcntb\m@ne\def\@citea{}%
  \@cite{\@for\@citeb:=#2\do%                                               for aech citation...
         {\edef\@citeb{\expandafter\@firstofone\@citeb}%                    eat trailing space
          \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi% write to aux
          \@ifundefined{b@\@citeb}%                                         if label undefined..
                       {\@citeo\@tempcntb\m@ne\@citea%                      ... then ...
                        \def\@citea{,\penalty\@m\ }{\reset@font\bf ?}%
	                \G@refundefinedtrue\@latex@warning%
                        {Citation `\@citeb' on page \thepage \space undefined}}%
                       {\setbox\z@\hbox{\global\@tempcntc0\csname %         ... else
                                        b@\@citeb\endcsname}%
                        \advance\@tempcntb\@ne%
                        \ifnum\@tempcntb=\@tempcntc%
                        \else\advance\@tempcntb\m@ne\@citeo%
                             \@tempcnta\@tempcntc\@tempcntb\@tempcntc
                        \fi%
                        }%
         }\@citeo}{#1}%
	 \if@draft\norm@note{CIT: }{#2}\fi			% **DRAFT**
    }% end definition of \@citex
%This really prints out the cit-numbers
\def\@citeo{\ifnum\@tempcnta>\@tempcntb%    
            \else\@citea\def\@citea{,\penalty\@m\ }%
                  \ifnum\@tempcnta=\@tempcntb%
                  \intJlink{\hash bib\the\@tempcnta}{\the\@tempcnta}% if there is no range
                  \else{\advance\@tempcnta\@ne%                 % if there is a range
                       \ifnum\@tempcnta=\@tempcntb%
                       \else\def\@citea{\,--\,}%
                       \fi%
                       \advance\@tempcnta\m@ne%
                       \intJlink{\hash bib\the\@tempcnta}{\the\@tempcnta}\@citea%first
                       \intJlink{\hash bib\the\@tempcntb}{\the\@tempcntb}}%last
                  \fi%
             \fi}
%%%%%%%%%%%%%%% until here %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------------------------------------------------------%
% CITATION TAGS ARE TOGETHER WITH BIB STUFF.
% CITATION HREF
\else             % w.r.t. \if@Jcits above
\def\@citex[#1]#2{%			% UNFORTUNATELY REDEFINED!!!!
  \let\@citea\@empty
  \@cite{\@for\@citeb:=#2\do
    {\@citea\def\@citea{,\penalty\@m\ }%
     \edef\@citeb{\expandafter\@firstofone\@citeb}%
     \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi
     \@ifundefined{b@\@citeb}{\mbox{\reset@font\bf ?}%
	\G@refundefinedtrue
	\@latex@warning
	  {Citation `\@citeb' on page \thepage \space undefined}}%
	{\edef\tmp@bn{\csname b@\@citeb\endcsname}%
	 \hbox{\intJlink{\hash bib\tmp@bn}{\tmp@bn}}}}}{#1}%		% **HYPER**
	 \if@draft\norm@note{CIT: }{#2}\fi			% **DRAFT**
	 }
\fi             % w.r.t. \if@Jcits above

%-----------------------------------------------------------------%
% LABEL, REF AND PAGEREF, TEXTREF, ~ COMPATIBLE:
\let\old@label\label						% OLD LATEX COMMAND.
\def\label{\bgroup\catcode`\>=15\catcode`\"=15 \catcode`\==15\@@label}		
\newcommand{\@@label}[1]{\egroup\name{ref-#1}%		% LABEL IN HYPER TAG.
			 \old@label{#1}%		% 
			 \if@draft%			% DRAFT:
			 \ifmmode\math@note{#1}%
			 \else\norm@note{}{LAB: #1}\fi%
			 \fi%
			 }
\if@hyper
\let\old@ref\ref \let\old@pageref\pageref		% OLD LATEX COMMANDS.
\renewcommand{\ref}[1]{\@ifundefined{r@#1}{}{\intJlink{\hash ref-#1}}%
		       {\old@ref{#1}}} % LABEL INSIDE HREF.
\renewcommand{\pageref}[1]{\@ifundefined{r@#1}{}{%	% UNDEFINED => NO HREF
	      \edef\tmp@ref{\noexpand\@secondoftwo\csname r@#1\endcsname}%
	      \intJlink{\hash pag\tmp@ref}}{\old@pageref{#1}}}
\fi
\newcommand{\textref}[2]{\@ifundefined{r@#1}
			{%
			\protect\G@refundefinedtrue
			\nfss@text{\reset@font\bf ?#2?}%
   			\@latex@warning{Reference `#1' on page \thepage \space
				             undefined}}
			{\vrule height \z@ width \z@\intJlink{\hash ref-#1}{#2}}}
%------------------------------------------------------------------%
%%%%%%%%%%%%%%%%%%%%%%%%%% END HYPER-STUFF %%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%% JINST HEADINGS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ps@JINST{% 			
    \def\@oddfoot{\ifnum\thepage=0\if@preprint\else
		\Jcopyright@box\fi\hfill % copyright only on front page of published papers
		\if@Jspecialurl\copy\Jspecial@url\else\if@preprint\else\copy\Jpaper@url\fi\fi %possible url
		\else\reset@font\hfil-- \thepage\ --\hfil\fi} % page numbers on other pages
    \if@draft\edef\cur@opt{\@curroptions}\fi
    \def\@oddhead{\name{pag\thepage}\hfil\if@draft\copy\drft@box\fi}
    \if@twoside\let\@evenhead\@oddhead\let\@evenfoot\@oddfoot\fi
    \let\@mkboth\@gobbletwo
    \let\sectionmark\@gobble
    \let\subsectionmark\@gobble
    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TITLE PAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\maketitle{\JINST@ignol{\maketitle}}
\newcommand\auto@maketitle{\begingroup
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \def\@makefnmark{\rlap{\@textsuperscript{\normalfont\@thefnmark}}}%
    \long\def\@makefntext##1{\parindent 1em\noindent
            \hb@xt@1.8em{\hss\@textsuperscript{\normalfont\@thefnmark}}##1}%
    \let\footnote\thanks%
	 \newpage				%
	 \@maketitle				% CALL ACTUAL FORMATTING
	 \@thanks				% TITLE THANKS
	 \thispagestyle{JINST} 
 	 \setcounter{page}\z@
	 \newpage				% FINE PAGINA
  \endgroup
  \setcounter{footnote}{0}%			
  \if@todotoc					% IF THERE IS A SECTION
      \noindent\rule\textwidth{.1pt}		% THEN MAKE TOC...
      \vskip 2em \@plus 3ex \@minus 3ex
      \tableofcontents
      \vskip 2em \@plus 3ex \@minus 3ex
      \noindent\rule\textwidth{.1pt}
      \vskip 2em \@plus 3ex \@minus 3ex
  \fi
  \if@preprint\else
      \gdef\tableofcontents{\JINST@igno{\tableofcontents\space is automatic}}
  \fi
  \global\let\thanks\@gobble
  \global\let\@maketitle\relax			%
  \global\let\@thanks\@empty			%
  \global\let\@author\@empty			% KILL ALL 
  \global\let\@date\@empty			%
  \global\let\@title\@empty			%
  \global\let\@abstract\@empty			%
  \global\let\title\relax			%
  \global\let\author\relax			%
  \global\let\date\relax			%
  \global\let\and\relax				%
  \global\let\email\@gobble
  \global\let\received\relax
  \global\let\revised\relax
  \global\let\accepted\relax
  \global\let\published\relax
  \global\let\JINSTcopydate\relax
  \global\let\Jspecialurl\relax
  \global\let\keywords\relax
  \global\let\endkeywords\relax
}
%%%%%%%%%%%%%%%%%%%%%%%%%% ACTUAL TITLEPAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newskip\titlesk@ja		% Skips for titlepage
\newskip\titlesk@jb		%
\newskip\titlesk@jc		%
\titlesk@ja= 1.6em plus .4fil%			% Before title 
\titlesk@jb= 2em   plus .06fil minus  .5ex%	% Between title/rule
\titlesk@jc= 2em   plus .05fil minus 1.2ex%	% Before authors

\def\@maketitle{%				% PAGE IS FLUSHED LEFT
\begin{flushleft}%				% PAY ATTENTION TO \par'S
% page with queries for authors in proof
\if@Jqueries
    \setcounter{page}{0}
\noindent{\let\thanks\@gobble\let\footnote\@gobble%
          \large\sffamily\@title\par}                     % title
\vskip.4\titlesk@jb
\noindent{\Large\sffamily\bfseries\queriesname\hfill\par} % queriesname
\vskip.7\titlesk@jb
    \hrule height 1\p@%            otherwise = 1.5pt.     % rule
\vskip.7\titlesk@jb
{\noindent\footnotesize Please reply to the following queries using
the appropriate tool ``{\sc send proofs}'' at the bottom of the
preprint page on \href{http://jinst.sissa.it}{\tt http://jinst.sissa.it}}
\vskip\titlesk@jc
\Jqueries@auth                                            % queries
    \newpage
    \setcounter{page}{0}
\fi
%header for preprints
\if@preprint					%%% PREPRINT HEADER: 
    \vskip-7em					%
    \underline{\tiny Preprint typeset 		%
                in JINST style -		        %
  		\if@hyper{HYPER VERSION}	%
		\else{PAPER VERSION}\fi } 	%
    \normalsize\hfill%				%
    \begin{tabular}[t]{r}\@preprint\end{tabular}%   % PREPRINT NUMBERS
\else						%
% header for published papers
    \vskip-7em\hfill
    {\small\scshape Published by Institute of Physics 
 	               Publishing and SISSA}
    \vskip-1.35\baselineskip\logo\hrulefill
    \vskip-1.5\baselineskip\hskip21.73\p@%	
    \hfill{\parbox[t]{30em}{\begin{flushright}\setlength\baselineskip{11pt}\footnotesize
				\Jrece@cs\\
				\if@revi\Jrevi@cs\\\fi
				\Jacce@cs\\
				\Jpubli@cs
			      \end{flushright}}}%
\fi\null
% end headers
\vskip \titlesk@ja		   % vspace before title
% TITLE large sans-serif bf
{\LARGE \sffamily\bfseries\@title\par}  
%
\vskip \titlesk@jb                 % vspace between title and rule
% RULE
\hrule height 1.5\p@%
%
\vskip \titlesk@jb		   % vspace between rule and authors
% AUTHORS\\ADDRESSES
\vskip-\auth@skip
{\normalsize \bfseries \sffamily \@author \par}
%
\vskip \titlesk@jc                 % vspace between authors and abstract
% ABSTRACT
\parbox\textwidth{\abstract@cs}%	
\normalsize                        % why reset size?
% KEYWORDS IF PRESENT
\if@keywords	
\vskip .9\titlesk@jc	   % vspace between abstract and keywords
\par
\@keywords				
\fi
% DEDICATION, IF PRESENT
\dedic@box				
\end{flushleft}%			% FINISHED.
}
%%%%%%%%%%%%%%%%%%%%%%%%%%% STANDARD STUFF %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setcounter{secnumdepth}{3}
\newcounter {part}
\newcounter {section}
\newcounter {subsection}[section]
\newcounter {subsubsection}[subsection]
\newcounter {paragraph}[subsubsection]
\newcounter {subparagraph}[paragraph]
\renewcommand\thepart         {\@Roman\c@part}
\renewcommand\thesection      {\@arabic\c@section}
\renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}
\renewcommand\thesubsubsection{\thesubsection.\@arabic\c@subsubsection}
\renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}
\renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}
%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTION FORMATS %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\secstyle{\bfseries}
\def\ts@flag{\let\d@t.%					% Sections get ``.''
	     \immediate\write\@auxout			% IF THERE IS A SECTION
	     {\string\global\string\@todotoctrue}}	% THEN SIGNAL IN AUX.

\newcommand\part{\par
   \addvspace{4ex}%
   \@afterindentfalse
   \secdef\@part\@spart}

\def\@part[#1]#2{\ts@flag
    \ifnum \c@secnumdepth >\m@ne
      \refstepcounter{part}%			% DAMN LATEX !!! BELOW,
      \addcontentsline{toc}{part}{\string\intJlink	% UNFORTUNATELY, NO NUMBERLINE:
				  {\string\hash\space part\the\c@part}%
				  {\thepart}\hspace{1em}#1}%
    \else
      \addcontentsline{toc}{part}{#1}%
    \fi
    {\parindent \z@ \raggedright
     \interlinepenalty \@M
     \normalfont
     \ifnum \c@secnumdepth >\m@ne
       \name{part\the\c@part}\Large\bfseries \partname~\thepart
       \par\nobreak
     \fi
     \huge \bfseries #2%
     \markboth{}{}\par}%
    \nobreak
    \vskip 3ex
    \@afterheading\let\d@t\relax}
\def\@spart#1{%
    {\parindent \z@ \raggedright
     \interlinepenalty \@M
     \normalfont
     \huge \bfseries #1\par}%
     \nobreak
     \vskip 3ex
     \@afterheading}

\newcommand\section{\@startsection{section}{1}{\z@}%
                                   {-3.5ex \@plus -1.3ex \@minus -.7ex}%
                                   {2.3ex \@plus.4ex \@minus .4ex}%
                                   {\normalfont\large\secstyle}}
\newcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {-2.3ex\@plus -1ex \@minus -.5ex}%
                                   {1.2ex \@plus .3ex \@minus .3ex}%
                                   {\normalfont\normalsize\secstyle}}
\newcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                   {-2.3ex\@plus -1ex \@minus -.5ex}%
                                   {1ex \@plus .2ex \@minus .2ex}%
                                   {\normalfont\normalsize\secstyle}}
\newcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                   {1.75ex \@plus1ex \@minus.2ex}%
                                   {-1em}%
                                   {\normalfont\normalsize\bfseries}}
\newcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
                                   {1.75ex \@plus1ex \@minus .2ex}%
                                   {-1em}%
                                   {\normalfont\normalsize\bfseries}}

% ---- turnaround for sections with figures ------ %
\def\bef@sec{\iffigprocessing\JINST@warnl{Floating figure \the\ffigcount\space
						and startsection colliding}\fi
	     \iftabprocessing\JINST@warnl{Floating table \the\ftabcount\space
						and startsection colliding}\fi
	     \edef\bef@everypar{\the\everypar}}	% HACK FOR FLOATS AND \everypar
\def\aft@sec{\let\d@t\relax			% RESTORE: NO DOTTED SUBSECS..
	     \edef\tmp@everypar{\the\everypar}% % DELETED CLUBPENALTY, BELOW.
	     \everypar\expandafter{\bef@everypar{\tmp@everypar}}}% RESTORE.
\let\old@sec\section				%
\let\old@ssec\subsection			%
\let\old@sssec\subsubsection			% OLD SECTIONING COMMANDS.
\let\old@par\paragraph				%
\let\old@spar\subparagraph			%
% ------- new forms ------- %
\renewcommand{\section}{\secdef\JINST@sec\JINST@secs}
\renewcommand{\subsection}{\secdef\JINST@ssec\JINST@ssecs}
\renewcommand{\subsubsection}{\secdef\JINST@sssec\JINST@sssecs}
\renewcommand{\paragraph}{\secdef\JINST@par\JINST@pars}
\renewcommand{\subparagraph}{\secdef\JINST@spar\JINST@spars}
% ---- unstarred forms ---- %
\def\JINST@sec[#1]#2{\ts@flag\bef@sec\old@sec[#1]{#2}\aft@sec}
\def\JINST@ssec[#1]#2{\bef@sec\old@ssec[#1]{#2}\aft@sec}
\def\JINST@sssec[#1]#2{\bef@sec\old@sssec[#1]{#2}\aft@sec}
\def\JINST@par[#1]#2{\bef@sec\old@par[#1]{#2}\aft@sec}
\def\JINST@spar[#1]#2{\bef@sec\old@spar[#1]{#2}\aft@sec}
% ----- starred forms ----- %
\def\JINST@secs#1{\bef@sec\old@sec*{#1}\aft@sec}
\def\JINST@ssecs#1{\bef@sec\old@ssec*{#1}\aft@sec}
\def\JINST@sssecs#1{\bef@sec\old@sssec*{#1}\aft@sec}
\def\JINST@pars#1{\bef@sec\old@par*{#1}\aft@sec}
\def\JINST@spars#1{\bef@sec\old@spar*{#1}\aft@sec}
% ----- end hack for sections with floats --------%

\if@twocolumn
  \setlength\leftmargini  {2em}
\else
  \setlength\leftmargini  {2.5em}
\fi
\leftmargin  \leftmargini
\setlength\leftmarginii  {2.2em}
\setlength\leftmarginiii {1.87em}
\setlength\leftmarginiv  {1.7em}
  \setlength\leftmarginv  {1em}
  \setlength\leftmarginvi {1em}
\setlength  \labelsep  {.5em}
\setlength  \labelwidth{\leftmargini}
\addtolength\labelwidth{-\labelsep}
\@beginparpenalty -\@lowpenalty
\@endparpenalty   -\@lowpenalty
\@itempenalty     -\@lowpenalty
\renewcommand\theenumi{\@arabic\c@enumi}
\renewcommand\theenumii{\@alph\c@enumii}
\renewcommand\theenumiii{\@roman\c@enumiii}
\renewcommand\theenumiv{\@Alph\c@enumiv}
\newcommand\labelenumi{\theenumi.}
\newcommand\labelenumii{(\theenumii)}
\newcommand\labelenumiii{\theenumiii.}
\newcommand\labelenumiv{\theenumiv.}
\renewcommand\p@enumii{\theenumi}
\renewcommand\p@enumiii{\theenumi(\theenumii)}
\renewcommand\p@enumiv{\p@enumiii\theenumiii}
\newcommand\labelitemi{$\m@th\bullet$}
\newcommand\labelitemii{\normalfont\bfseries --}
\newcommand\labelitemiii{$\m@th\ast$}
\newcommand\labelitemiv{$\m@th\cdot$}
\newenvironment{description}
               {\list{}{\labelwidth\z@ \itemindent-\leftmargin
                        \let\makelabel\descriptionlabel}}
               {\endlist}
\newcommand*\descriptionlabel[1]{\hspace\labelsep
                                \normalfont\bfseries #1}
%%%%%%%%%%%%%%%%%%%%%%%%%% AUTHORS/ADDRESSES %%%%%%%%%%%%%%%%%%%%%%%%%%
% *** After proceedings, the authors go in a hbox. => \break does not work!!
% *** if no address nobody closes the box!
\newif\if@speaker\@speakerfalse
\newif\if@dblspeak\@dblspeakfalse
\newtoks\prev@t
\newtoks\cur@t
\newbox\@firstaubox
\newskip\addr@skip\addr@skip=.6em\@plus.02fil\@minus.3ex %\fi
\newskip\auth@skip\auth@skip=.6em\@plus.03fil\@minus.2ex %\fi
\renewcommand\@author{\parskip\z@
		      \def\\{\egroup			% CLOSE & aftergroup!
			\par				% FIRST TIME \\=>ADDR.
			\vskip\addr@skip		% GLUE UNDER AUTHOR
			\hskip1em%			% ADDRESS INDENT
			\vbox\bgroup\hsize=.9\textwidth	% 
			\small\it\raggedright		% STYLE FOR ADDRESSES
			\def\\{\par\leavevmode\ignorespaces}%\let\\\relax%
			\leavevmode\ignorespaces}%
			}
\renewcommand\author[1]{%
		\global\@authortrue			%
		\prev@t=\expandafter{\@author}%		% TWO TOKEN LISTS.
		\cur@t={\vskip\auth@skip		% glue before auth.
			\vtop\bgroup #1\egroup		% ACTUAL AUTH.\\ADD.
			\par}%				%
		\long\xdef\@author{\the\prev@t\the\cur@t}%STORE ALL IN \@AUTHOR
		}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RECEIVED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\received[1]{\gdef\Jrece@cs{{\scshape\receivedname} 
                                       {\itshape #1}}\@recetrue\let\received\gobble}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% REVISED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\revised[1]{\gdef\Jrevi@cs{{\scshape\revisedname}
                                      {\itshape #1}}\@revitrue\let\revised\gobble}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ACCEPTED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\accepted[1]{\gdef\Jacce@cs{{\scshape\acceptedname}
                                       {\itshape #1}}\@accetrue\let\accepted\gobble}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PUBLISHED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\published[1]{\gdef\Jpubli@cs{{\scshape\publishedname}
                                       {\itshape #1$\vphantom{,}$}}\@publitrue\let\published\gobble}
%%%%%%%%%%%%%%%%%%%%%%%%%% COPYRIGHT DATE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\Jcopy@date
\newcommand\JINSTcopydate[1]{\global\setbox\Jcopy@date
                        \hbox{\scriptsize #1}\global\@Jcopytrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DEDICATED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\dedic@box{\relax}
\newcommand\dedicated[1]{\gdef\dedic@box{\vskip2em minus 1.2ex
                              \vbox{\small\it\raggedleft #1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% QUERIES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if@Jqueries\@Jqueriesfalse
\gdef\Jqueries@auth{\relax}
\newcommand\QueriesForAuth[1]{\@Jqueriestrue\gdef\Jqueries@auth{%
                              {\raggedright #1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%% ACKNOWELEDGMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\acknowledgments{\section*{\acknowlname}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EMAIL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\email[1]{{\tt\href{mailto:#1}{#1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PREPRINT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\@preprint\relax
\newcommand\preprint[1]{\long\gdef\@preprint{#1}} 
%%%%%%%%%%%%%%%%% SPECIAL URL overrides paper@url %%%%%%%%%%%%%%%%%%%%%
\newbox\Jspecial@url
\newcommand\Jspecialurl[1]{\global\setbox\Jspecial@url\hbox{\tiny\ttfamily
			#1}\@Jspecialurltrue}
%%%%%%%%%%%%%%%%%%%%%%%%% FILE NAME AND URL %%%%%%%%%%%%%%%%%%%%%%%%%%%
%\global\newbox\Jacce@month
%\global\newcount\Jacce@year
%\global\newbox\Jacce@number
%\def\Jsplit@ident#1(#2)#3.{\global\setbox\Jacce@month\hbox{\tiny\ttfamily #1}
%			  \global\Jacce@year= #2
%			  \global\setbox\Jacce@number\hbox{\tiny\ttfamily #3}

%\gdef\Jfile@name{\hbox{\tiny\ttfamily
%		jinst\unhcopy\Jacce@month\the\Jacce@year\unhcopy\Jacce@number}}

\newbox\Jpaper@url
\global\setbox\Jpaper@url\hbox{\tiny\ttfamily http://www.iop.org/EJ/jinst/}
                              %\Jfile@name/\Jfile@name.pdf}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COPYRIGHT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\Jcopyright@box{\hbox{\if@preprint\else{\scriptsize $\copyright$
		\if@Jcopy\unhbox\Jcopy@date\else\the\year\fi\ IOP Publishing Ltd\ and SISSA}\fi}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ABSTRACT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% *** For beton! We need a cs, not a box. Maybe also for refs.. %%%%%%

\newcommand{\abstract}[1]%		% ABSTR. IN NORMALSIZE
	{\gdef\abstract@cs{		% cs FOR WHOLE ABSTRACT
	{\noindent{\scshape\abstractname}\ \ignorespaces #1}}
	 \normalsize
	 \global\@abstracttrue\let\abstract\gobble}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% KEYWORDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@keywords{\relax}%                   % CS FOR WHOLE KEYWORDS
\def\keywords{\bgroup\gdef\@comma{,}\catcode`\ =\active\catcode`,=\active
		\@@keywords}
\begingroup
\catcode`\ =\active\catcode`,=\active\global
\def\@@keywords#1{\gdef\@keywords{\noindent{\scshape\keywordsname}
		\bgroup\def, {+}\def {_}%	%ATTENTION: NO EXPANSION.
		%\href{http://jinst.sissa.it/stdsearch}%
						{\let,\@comma\let \ #1}.
		\egroup}\egroup\global\@keywordstrue\let\keywords\gobble}%
\endgroup
%%%%%%%%%%%%%%%%%%%%%%%%%% OTHER ENVIRONMENTS %%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{verse}
               {\let\\\@centercr
                \list{}{\itemsep      \z@
                        \itemindent   -1.5em%
                        \listparindent\itemindent
                        \rightmargin  \leftmargin
                        \advance\leftmargin 1.5em}%
                \item\relax}
               {\endlist}
\newenvironment{quotation}
               {\list{}{\listparindent 1.5em%
                        \itemindent    \listparindent
                        \rightmargin   \leftmargin
                        \parsep        \z@ \@plus\p@}%
                \item\relax}
               {\endlist}
\newenvironment{quote}
               {\list{}{\rightmargin\leftmargin}%
                \item\relax}
               {\endlist}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if@twothms\@twothmsfalse

\if@preprint%\ifx\@thmcountersep\@undefined
%\def\@xthm#1#2{\@begintheorem{#2}{\csname the#1\endcsname.}\ignorespaces}% after thm number
\else									 % if published 
\def\@xthm#1#2{\@begintheorem{#2\if@twothms\else.\fi}			 % theorems are numbered
		{\if@twothms\csname the#1\endcsname.\fi}		 % only if more than one
		\ifnum \csname the#1\endcsname>1 \immediate\write\@auxout% and not within sections
				{\string\global\string\@twothmstrue}\fi
		\ignorespaces}
\fi

\newcommand\Proof{\noindent\emph{Proof.}\ }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\appendix{\par
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \renewcommand\thesection{\@Alph\c@section}}

%%%%%%%%%%%%%%%%%%%%%%%%%%% SOME MORE LENGHTS %%%%%%%%%%%%%%%%%%%%%%%%%
\setlength\arraycolsep{2\p@}		% TO MATCH eqnarrays<->equations
\setlength\tabcolsep{6\p@}
\setlength\arrayrulewidth{.4\p@}
\setlength\doublerulesep{2\p@}
\setlength\tabbingsep{\labelsep}
\skip\@mpfootins = \skip\footins
\setlength\fboxsep{3\p@}
\setlength\fboxrule{.4\p@}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THE EQUATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\theequation{\ifnum\c@section=0\else\thesection.\fi
			  \@arabic\c@equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIGURES, TABLES %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{figure}
\renewcommand\thefigure{\@arabic\c@figure}
\def\fps@figure{Htbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{\figurename~\thefigure}
\newenvironment{figure}
               {\@float{figure}}
               {\end@float}
\newenvironment{figure*}
               {\@dblfloat{figure}}
               {\end@dblfloat}
\newcounter{table}
\renewcommand\thetable{\@arabic\c@table}
\def\fps@table{tbp}
\def\ftype@table{2}
\def\ext@table{lot}
\def\fnum@table{\tablename~\thetable}
\newenvironment{table}
               {\@float{table}}
               {\end@float}
\newenvironment{table*}
               {\@dblfloat{table}}
               {\end@dblfloat}
%%-----------------------------------------------------------------%%
\newcommand{\FIGURE}[2][v]{\begin{floatingfigure}[#1]#2
                                        \end{floatingfigure}}
\newcommand{\TABLE}[2][v]{\begin{floatingtable}[#1]{#2}
                                        \end{floatingtable}}
\newcommand{\EPSFIGURE}[3][v]{\begin{floatingfigure}[#1]\epsfig{file=#2}
                                        \caption{#3}\end{floatingfigure}}
\newcommand{\TABULAR}[4][v]{\begin{floatingtable}[#1]{\begin{tabular}{#2}
					#3\end{tabular}}\caption{#4}
                                        \end{floatingtable}}
%Check below, and put automatic width ***
\newcommand{\DOUBLEFIGURE}[5][ht]{\@dblfloat{figure}[#1]\centerline{%
		\parbox{.45\textwidth}{\centerline{\epsfig{file=#2}}}~~~~
		\parbox{.45\textwidth}{\centerline{\epsfig{file=#3}}}}
		\centerline{\parbox[t]{.45\textwidth}{\caption{#4}}~~~~
		\parbox[t]{.45\textwidth}{\caption{#5}}}\end@dblfloat}
\newcommand{\DOUBLETABLE}[5][ht]{\@dblfloat{table}[#1]\centerline{%
		\parbox{.45\textwidth}{\centerline{#2}}~~~~
		\parbox{.45\textwidth}{\centerline{#3}}}
		\centerline{\parbox[t]{.45\textwidth}{\caption{#4}}~~~~
		\parbox[t]{.45\textwidth}{\caption{#5}}}\end@dblfloat}
%%%%%%---------------- FROM FLOATFLT PACKAGE ------------------%%%%%%%%
%% Original file `floatflt.sty', modified by F.Nesti <nesti@sissa.it> to:
%% be inserted in JINST.cls;
%% correct float placement when shifting past pages;
%% correct incompatibility with \marginpar;
%% correct incompatibility with \@startsection;
%% correct persisting indentation in following pars;
%% let float also at beginning of pages; 
%% avoid the widht specification.
%% 
%% Original was 1994-1996 by Mats Dahlgren <matsd@physchem.kth.se>. 
%% 
%%%%%%%%\NeedsTeXFormat{LaTeX2e}[1994/06/01]		%LEFT THIS STUFF TO 
%%%%%%%%\ProvidesPackage{floatflt}[1996/02/27 v. 1.3]	%RECONVERT TO PACKAGE.
\newcounter{OptionTest}
\if@twoside
 \setcounter{OptionTest}{0}
\else							% POS: 2side=p/1side=r
 \setcounter{OptionTest}{1}
\fi
%%%%%%%%\DeclareOption{rflt}{\setcounter{OptionTest}{1}}
%%%%%%%%\DeclareOption{lflt}{\setcounter{OptionTest}{2}} % CHOSEN.
%%%%%%%%\DeclareOption{vflt}{\setcounter{OptionTest}{0}}
%%%%%%%%\DeclareOption*{\OptionNotUsed}
%%%%%%%%\ProcessOptions
\newbox\@tmpbox
\newbox\figbox
\newbox\tabbox
\newbox\pagebox
\newcount\ffigcount
\newcount\ftabcount
\newcount\hangcount
\newcount\nosuccesstryfig
\newcount\nosuccesstrytab
\newdimen\figgutter   \figgutter=1truepc
\newdimen\tabgutter   \tabgutter=1truepc
\newdimen\fl@wd
\newdimen\fl@ht
\newdimen\htdone      \htdone=\z@
\newdimen\pageht
\newdimen\startpageht
\newdimen\floatfltwidth
\newdimen\fltitemwidth
\newif\iftryingfig     \tryingfigfalse
\newif\iftryingtab     \tryingtabfalse
\newif\ifdoingfig      \doingfigfalse
\newif\ifdoingtab      \doingtabfalse
\newif\iffigprocessing \figprocessingfalse
\newif\iftabprocessing \tabprocessingfalse
\newif\ifpageafterfig  \pageafterfigfalse
\newif\ifpageaftertab  \pageaftertabfalse
\newif\ifoddpages
\newif\ifoutput
\newtoks\outputpretest
\def\@captype{}
%%---------------- ORRIBLE HACKS, SORRY -------------------------%%
\let\old@marginpar\marginpar				% 
\renewcommand\marginpar[1]{{\outputpretest={\outputtrue}% REDEF \marginpar.
			    \old@marginpar{#1}}}	%
\def\g@addto#1#2{{\toks@\expandafter{#1#2}%
		  \xdef#1{\the\toks@}}}%
\def\postpone@captions{%			%
	\global\let\tmp@caption\caption		% \label, LATER.
	\global\let\later@capt\relax		% UN PO' PESANTI 
	\gdef\later@label{}%			% MA D'ALTRONDE...
	\let\J@ref\ref\def\ref{\protect\J@ref}% % protect ref in captions.. 
	\renewcommand\caption{\@ifnextchar[\J@@caption\J@caption}%
	\newcommand\J@caption[1]{\gdef\later@capt{\tmp@caption{##1}}}% LOCAL!!
	\newcommand\J@@caption[2][v]%
				{\gdef\later@capt{\tmp@caption[##1]{##2}}}% LOCAL!!
	\renewcommand\@@label[1]{\egroup\name{ref-##1}%	% TAG WHERE CALLED, AT LEAST,
			       \if@draft\norm@note{}{LAB: ##1}\fi% & DRAFTNOTE.
			       \g@addto\later@label{\old@label{##1}}}%
			}
\AtEndDocument{\iftryingfig\JINST@warnl{Floating figure \the\ffigcount\space
					remains undone}\fi
		\iftryingtab\JINST@warnl{Floating table \the\ftabcount\space
					remains undone}\fi} 
%%----------------- FIGURE ---------------------------------------%%
\newenvironment{floatingfigure}[1][v]%
{\@tfor \@tempa :=#1\do {\xdef\@fside{\@tempa}}%
 \global\advance\ffigcount by 1%
 \iffigprocessing {\count0=\ffigcount\advance\count0 by -1%
   		   \JINST@warnl{Floating figures \the\count0\space\space and
       			\the\ffigcount\space colliding}}\fi
 \iftabprocessing  \JINST@warnl{Floating table \the\ftabcount\space and 
			floating figure \the\ffigcount\space colliding}\fi
 \postpone@captions
 \global\setbox\@tmpbox=\hbox\bgroup% begin of figbox %HBOX FOR AUTO WIDTH!
}
{%
\egroup%				% CALCULATE WIDTH (NO CAPTION FOR NOW)
\global\setlength{\floatfltwidth}{\the\wd\@tmpbox}%
% New behavior:	wd < .6 columnwidth => floatflt.
%		wd < columnwidth    => float{figure}
%		wd > columnwidth    => dblfloat{figure}
\ifdim\floatfltwidth<.6\columnwidth%	% IF NOT TOO WIDE OK:
 \global\setbox\figbox=\vbox{\hsize=\floatfltwidth
			     \def\@captype{figure}%
			     \noindent\unhbox\@tmpbox
			     \later@capt\later@label}%
 \global\figprocessingtrue
 \global\everypar={\tryfig\oldeverypar}% must be set globally!
 \figinsert\par
\else%					% ELSE NORMAL LATEX FIGURE, SIGH.
% \JINST@mess{Floating figure \the\ffigcount\space is 
%			wide becomes a LaTeX float}%
 \if\@fside v \def\@fside{ht}\fi
 \ifdim\floatfltwidth<\columnwidth
    \def\@@tempa{\@float{figure}[}\let\@@tempb\end@float
 \else
    \def\@@tempa{\@dblfloat{figure}[}\let\@@tempb\end@dblfloat
 \fi
 \expandafter\@@tempa\@fside]\center\unhbox\@tmpbox\later@capt\later@label\@@tempb
\fi
}
%%------------ TABLE ----------------------------------------------%%
\newenvironment{floatingtable}[1][v]%
{\@tfor \@tempa :=#1\do {\global\edef\@tside{\@tempa}}%
 \global\advance\ftabcount by 1%
 \iftabprocessing {\count0=\ftabcount\advance\count0 by -1%
     		   \JINST@warnl{Floating tables \the\count0\space
            		\space and \the\ftabcount \space colliding}}\fi
 \iffigprocessing  \JINST@warnl{Floating figure \the\ffigcount\space and 
			floating table \the\ftabcount\space colliding}\fi
 \postpone@captions
 \global\setbox\@tmpbox=\hbox\bgroup% begin of tabbox, ACTUALLY AN HBOX.
}
{%
\egroup% end of \tabbox, 		% ACTUALLY \@tmpbox
\global\setlength{\floatfltwidth}{\the\wd\@tmpbox}%
\ifdim\floatfltwidth<.6\columnwidth%	% IF NOT TOO WIDE OK:
  \global\setbox\tabbox=\vbox{\hsize=\floatfltwidth
			     \def\@captype{table}%
			     \noindent\unhbox\@tmpbox
			     \later@capt\later@label}%
  \global\tabprocessingtrue
  \global\everypar={\trytab\oldeverypar}%
  \tabinsert\par%
\else%					% ELSE NORMAL LATEX TABLE.
%  \JINST@mess{Floating table \the\ftabcount\space is 
%			wide becomes a LaTeX float}%
  \ifdim\floatfltwidth<1.1\columnwidth
    \if\@tside v \def\@tside{ht}\fi
    \def\@@tempa{\@float{table}[}\let\@@tempb\end@float
  \else
    \if\@tside v \def\@tside{t}\fi
    \def\@@tempa{\@dblfloat{table}[}\let\@@tempb\end@dblfloat
  \fi
  \expandafter\@@tempa\@tside]%		% ACTUALLY CALL THE LATEX FLOAT
  \center\unhbox\@tmpbox\later@capt\later@label
  \@@tempb
\fi%
}
%----------- prepare for tries ----------------------------%
\def\figinsert{%
   \global\nosuccesstryfig=0%
   \global\outputpretest={\do@test}%
   \global\tryingfigtrue \global\doingfigfalse%
   \global\pageafterfigfalse}%
\def\tabinsert{%
   \global\nosuccesstrytab=0%
   \global\outputpretest={\do@test}%
   \global\tryingtabtrue \global\doingtabfalse%
   \global\pageaftertabfalse}%
%----------- init -----------------------------------------%
\AtBeginDocument{%
 \edef\oldoutput{\the\output}
 \output={\the\outputpretest\ifoutput\oldoutput\fi}%
 \outputpretest={\outputtrue}%
 \edef\oldeverypar{\the\everypar}% PERCHE' NESSUNO LO RIMETTE PIU' A POSTO?***
}
%---- tests during \outputpretest -------------------------%
\def\do@test{%
   \ifnum\outputpenalty=-10005
%	\output
     \setbox\pagebox=\vbox{\unvbox255}%
     \global\pageht=\ht\pagebox
     \global\outputfalse
     \unvbox\pagebox
     \dimen0=\pageht\advance\dimen0 by 2 \baselineskip
     \ifdim\dimen0>\vsize\pagebreak[4]\global\pageht\z@\fi
   \else
     \global\outputtrue
     \ifnum\outputpenalty>-\@Mi			%ie \marginpar's give penalty.
	\ifdoingtab\global\pageaftertabtrue\fi
	\ifdoingfig\global\pageafterfigtrue\fi
     \fi
   \fi}%
%-------- check for side ----------------------------------%
\def\chk@side#1{% DEFINED \fl@sid, BUT IF CHOSEN A DEFAULT, ELIMINATE ALL ***
	{\edef\fl@sid{#1}%
	  \if\fl@sid r\global\oddpagestrue\fi
          \if\fl@sid l\global\oddpagesfalse\fi
          \if\fl@sid p%
              \ifodd\c@page\global\oddpagesfalse
                \else\global\oddpagestrue\fi
          \fi
          \if\fl@sid v%
             \ifnum\theOptionTest=0%
                 \ifodd\c@page\global\oddpagesfalse
                   \else\global\oddpagestrue\fi
             \else
                  \ifodd\theOptionTest\global\oddpagestrue
                    \else\global\oddpagesfalse\fi
             \fi
          \fi
         }}%
%-------- get point in page -------------------------------%
\def\get@pageht{{\everypar={\relax}\setbox0=\lastbox
       		\parindent=\wd0 \parskip=\z@ \par
         	\penalty-10005 \leavevmode}}%
%-------- try at everypar ---------------------------------%
\def\tryfig{%
	\global\fl@ht\ht\figbox
	\global\fl@wd\wd\figbox
	\global\let\fl@gut\figgutter
      \iftryingfig
	\get@pageht
	\dimen0=\vsize
	\advance\dimen0 by -\pageht
	\advance\dimen0 by -2\baselineskip
	\ifdim\dimen0>\fl@ht
	  \chk@side\@fside
	  \dimen0=0.3\baselineskip
	  \vrule depth \dimen0 width \z@%height 1.5\baselineskip
	  \vadjust{\kern -\dimen0
	  \vtop to \dimen0{%
             \baselineskip=\dimen0
             \vss \vbox to 1ex{%
             \ifoddpages
               \hb@xt@\hsize{\hss\copy\figbox}%
             \else% leftsetting
               \hb@xt@\hsize{\copy\figbox\hss}%
             \fi
             \vss}\null}}%
	  \global\tryingfigfalse
	  \global\doingfigtrue
	  \global\startpageht=\pageht
	  \global\htdone=\z@
	  \dohang
	  \ifnum\nosuccesstryfig>0%
	   \JINST@mess{Flt. fig. \the\ffigcount\space set on page \the\count0, 
	 		shifted \the\nosuccesstryfig\space par(s) forward}%
%	  \else
%	   \JINST@mess{Floating figure \the\ffigcount\space 
%			set on page \the\count0}%
	  \fi
	\else
          \global\advance\nosuccesstryfig by 1
	\fi
      \else%				% IF NOT TRYING
	\ifdoingfig
	  \get@pageht
	  \global\htdone=\pageht
	  \global\advance\htdone by -\startpageht
	  \ifpageafterfig
	    \global\doingfigfalse% IN CASE A PAGEBREAK JUST BELOW?
	  \else
	    \dimen0=\fl@ht
	    \advance\dimen0 by .85\baselineskip	% .85 ENOUGH: WE ARE AT NEW PAR
%	    \typeout{FLOAT HT: \the\dimen0, HTDONE: \the\htdone}
	    \ifdim\htdone<\dimen0%
		\dohang
	    \else
		\global\doingfigfalse
	    \fi
	  \fi
	  \ifdoingfig\else\global\figprocessingfalse\fi% IF NO MORE DOING.
	\else
	  \global\outputpretest={\outputtrue}% NOT RESTORE EVPAR IF NOT DOING?
	\fi%			% END IF DOING
      \fi%			% END IF TRYING
}
\def\trytab{%
	\global\fl@ht\ht\tabbox
	\global\fl@wd\wd\tabbox
	\global\let\fl@gut\tabgutter
       \iftryingtab
	\get@pageht
       \dimen0=\vsize
       \advance\dimen0 by -\pageht
       \advance\dimen0 by -2\baselineskip
       \ifdim\dimen0>\fl@ht
	 \chk@side\@tside
         \dimen0=0.3\baselineskip
         \vrule depth \dimen0 width \z@
         \vadjust{\kern -\dimen0
         \vtop to \dimen0{%
             \baselineskip=\dimen0
             \vss \vbox to 1ex{%
             \ifoddpages
               \hb@xt@\hsize{\hss\copy\tabbox}%
             \else% leftsetting
               \hb@xt@\hsize{\copy\tabbox\hss}%
             \fi
             \vss}\null}}%
       \global\tryingtabfalse
       \global\doingtabtrue
       \global\startpageht=\pageht
       \global\htdone=\z@
       \dohang
       \ifnum\nosuccesstrytab>0%
	\JINST@mess{Flt. tab. \the\ftabcount\space set on page \the\count0, 
			shifted \the\nosuccesstrytab\space par(s) forward}%
%       \else
%	\JINST@mess{Floating table \the\ftabcount\space 
%			set on page \the\count0}%
       \fi
     \else
       \global\advance\nosuccesstrytab by 1
     \fi
     \else
     \ifdoingtab
       \get@pageht
    \global\htdone=\pageht
    \global\advance\htdone by -\startpageht
    \ifpageaftertab
      \global\doingtabfalse
    \else
      \dimen0=\fl@ht
      \advance\dimen0 by .85\baselineskip	% .85 ENOUGH: WE ARE AT NEW PAR
      \ifdim\htdone<\dimen0%
         \dohang
      \else
         \global\doingtabfalse
      \fi
    \fi
    \ifdoingtab\relax\else\global\tabprocessingfalse\fi
  \else
    \global\outputpretest={\outputtrue}%
  \fi
\fi
}
%----- hanging lord -----------------------------%
\def\dohang{%
   \dimen0=\fl@ht
   \advance\dimen0 by -\htdone
   \advance\dimen0 by 1.999\baselineskip	% (16/12/98) WAS 1.49 BUT
   \hangcount=\dimen0				% TEX ROUNDS ON STRICT INTEGERS
   \divide\hangcount by \baselineskip		% IN THIS DIVISION!
%	\typeout{HANGCOUNT: \the\hangcount.}
%   \ifnum\hangcount > 0	% IF ZERO ALSO INDENT MUST BE NULL. (7/6/97)
     \dimen0=\fl@wd
     \advance\dimen0 by \fl@gut
     \ifoddpages
       \global\hangindent=-\dimen0% placing right
     \else 
       \global\hangindent=\dimen0% placing left
     \fi
   \global\hangafter=-\hangcount
%   \fi
}
%----------------------- TWO NEWITEMS ---------------------%
\newcommand{\fltitem}[2][\z@]{\setlength{\fltitemwidth}{\linewidth}%
  \addtolength{\fltitemwidth}{-\floatfltwidth}%
  \addtolength{\fltitemwidth}{-0.5em}%
  \item \parbox[t]{\fltitemwidth}{#2}\\[#1]}
\newcommand{\fltditem}[3][\z@]{\setlength{\fltitemwidth}{\linewidth}%
  \addtolength{\fltitemwidth}{-\floatfltwidth}%
  \addtolength{\fltitemwidth}{-0.5em}%
  \item[#2] \parbox[t]{\fltitemwidth}{#3}\\[#1]}
%%%%%%\endinput
%%% 
%%% End of ex-file `floatflt.sty'.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAPTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength\abovecaptionskip
\newlength\belowcaptionskip
\setlength\abovecaptionskip{8\p@}
\setlength\belowcaptionskip{0\p@}
\long\def\@makecaption#1#2{%
  \if@hyper{\edef\@pippo{the\@captype}
            \name{\@captype\expandafter\csname\@pippo\endcsname}}\fi%
  \vskip\abovecaptionskip
 {\let\label\@gobble%                           % FN 10.2.97 REMOVED LATEX BUG:
  \let\index\@gobble%                           % LARGE CAPTIONS PROCESS LABEL
  \let\glossary\@gobble%                        % TWO TIMES.
  \sbox\@tempboxa{\small {\bfseries #1.} #2}%   %
  \global\dimen0\wd\@tempboxa}%                 %
  \ifdim \dimen0 >\hsize
    \small {\bfseries #1.} #2\par
  \else
    \global\@minipagefalse \sbox\@tempboxa{\small {\bfseries #1.} #2}%
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FONTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
\DeclareRobustCommand*\mit{\@fontswitch\relax\mathnormal}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TOC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\tocsecs{}
\newcommand\@pnumwidth{1.55em}
\newcommand\@tocrmarg{2.55em}
\newcommand\@dotsep{4.5}
\setcounter{tocdepth}{3}
\newcommand\tableofcontents{%
    \section*{\contentsname\label{-TOC-}}
    \@starttoc{toc}%
    \gdef\tableofcontents{\JINST@igno{\tableofcontents\space already done}}}
\newcommand*\l@part[2]{\def\hyp@typ{part}%	
  \ifnum \c@tocdepth >-2\relax
    \addpenalty\@secpenalty
    \addvspace{2.25em \@plus\p@}%
    \begingroup
      \setlength\@tempdima{3em}%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      {\leavevmode
       \large \bfseries \tocsecs#1\hfil \hb@xt@\@pnumwidth{\hss
		\intJlink{\hash pag#2}{#2}}}\par
       \nobreak
       \if@compatibility
         \global\@nobreaktrue
         \everypar{\global\@nobreakfalse\everypar{}}%
      \fi
    \endgroup
  \fi}
\newcommand*\l@section[2]{\def\hyp@typ{sec}%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{1.0em \@plus\p@}%
    \setlength\@tempdima{1.8em}%	%WIDTH OF SECT. N.
    \begingroup
      \let\d@t.%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
        \tocsecs#1\nobreak\hfil %HREF HERE WOULD GET ALSO THE TITLE(...)
        \nobreak\hb@xt@\@pnumwidth{\hss \intJlink{\hash pag#2}{#2}}\par
    \endgroup
  \fi}

\newcommand*\l@subsection{\def\hyp@typ{sec}\@tocline{2}{1.8em}{2.3em}}
\newcommand*\l@subsubsection{\def\hyp@typ{sec}\@tocline{3}{4.1em}{3.1em}}
\newcommand*\l@paragraph{\def\hyp@typ{sec}\@tocline{4}{7.2em}{4.3em}}
\newcommand*\l@subparagraph{\def\hyp@typ{sec}\@tocline{5}{10.5em}{5em}}

\if@hyper
  \let\old@dtl\@dottedtocline
  \def\@dottedtocline#1#2#3#4#5{\old@dtl{#1}{#2}{#3}{#4}{%
						\intJlink{\hash pag#5}{#5}}}
\fi

\def\@tocline#1#2#3#4#5{%
  \ifnum #1>\c@tocdepth \else
    \vskip \z@ \@plus.2\p@
    {\leftskip #2\relax \rightskip \@tocrmarg \parfillskip -\rightskip
     \parindent #2\relax\@afterindenttrue
     \interlinepenalty\@M
     \leavevmode
     \@tempdima #3\relax
     \advance\leftskip \@tempdima \null\nobreak\hskip -\leftskip
     {#4}\nobreak
     \hfill
     \nobreak
     \hb@xt@\@pnumwidth{\hfil\normalfont \normalcolor \intJlink{\hash pag#5}{#5}}%
     \par}%
  \fi}


%%%%%%%%%%%%%%%%%%%%%% LIST OF FIGURES AND TABLES %%%%%%%%%%%%%%%%%%%%%
\if@draft			% ONLY IF DRAFT! ... 
 \newcommand\listoffigures{%
     \section*{\listfigurename
       \@mkboth{\MakeUppercase\listfigurename}%
               {\MakeUppercase\listfigurename}}%
     \@starttoc{lof}%
     }
 \newcommand*\l@figure{\def\hyp@typ{figure}\@dottedtocline{1}{1.5em}{2.3em}}
 \newcommand\listoftables{%
     \section*{\listtablename
       \@mkboth{%
           \MakeUppercase\listtablename}{\MakeUppercase\listtablename}}%
     \@starttoc{lot}%
     }
 \newcommand*\l@table{\def\hyp@typ{table}\@dottedtocline{1}{1.5em}{2.3em}}
\else
 \newcommand\listoffigures{\JINST@ignol{List of figures (draft mode only)}}
 \newcommand\listoftables{\JINST@ignol{List of tables (draft mode only)}}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BIBLIOGRAPHY %%%%%%%%%%%%%%%%%%%%%%%%%%%%***
\newdimen\bibindent
\setlength\bibindent{1.5em}
\newenvironment{thebibliography}[1]%	%UNFORTUNATELY MODIFIED..
     {\bgroup\raggedright\small\section*{\refname
        \@mkboth{\MakeUppercase\refname}{\MakeUppercase\refname}}%
      \list{\name{bib\@arabic\c@enumiv}% HOPE!
	    \@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy\clubpenalty4000\widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist\egroup}
\newcommand\newblock{\hskip .11em\@plus.33em\@minus.07em}
\if@draft
 \let\old@bbt\@bibitem\let\old@lbbt\@lbibitem% LOOK THE DISASTER HERE BELOW.
 \def\@lbibitem[#1]#2{\old@lbbt[#1]{#2}\reversemarginpar{\sf\bfseries\small#2}}
 \def\@bibitem#1{\old@bbt{#1}\reversemarginpar{\sf\bfseries\small#1}}
\fi
\let\@openbib@code\@empty
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% JOURNALS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@spires#1{\href{http://www-spires.slac.stanford.edu/spires/find/hep/www?j=#1}} 
%                               	%PITY THAT target IS NOT IMPLEMENTED.
\catcode`\%=12
\catcode`\|=14
|%%%% SM publications
\newcommand\jcap[3]  {\href{http://www.iop.org/EJ/abstract/1475-7516/#2/#1/#3}
		{{\it JCAP }{\bf #1} (#2) #3}}
\newcommand\jhep[3]  {\href{http://www.iop.org/EJ/abstract/1126-6708/#2/#1/#3}
		{{\it JHEP }{\bf #1} (#2) #3}}
\def\splitJINST#120#2#3#4#5#6#7#8#9{\href{http://www.iop.org/EJ/abstract/1748-0221/#1/#5#6/#4#5#6#7#8#9}
		{20#2#3 {\it JINST }{\bf #1} #4#5#6#7#8#9}}
\newcommand\jinst[3]   {\splitJINST#1#2#3}
                  
\def\splitJSTAT 20#1#2#3#4#5#6#7#8{\href{http://www.iop.org/EJ/abstract/1742-5468/20#1#2/#4#5/#3#4#5#6#7#8}
		{{\it J. Stat. Mech.\ }(20#1#2) #3#4#5#6#7#8}}
\newcommand\jstat[2]{\splitJSTAT#1#2}
\newcommand\pos[1]{\href{http://pos.sissa.it/cgi-bin/reader/contribution.cgi?id=#1}{\tt #1}}
|%%%% APS journals
\newcommand\pr[3]{\href{http://dx.doi.org/10.1103/PhysRev.#1.#3}
  {\emph{Phys.\ Rev.} {\bf #1} (#2) #3}}
\newcommand\pra[3]{\href{http://dx.doi.org/10.1103/PhysRevA.#1.#3}
  {\emph{Phys.\ Rev.} {\bf A #1} (#2) #3}}
\newcommand\prb[3]{\href{http://dx.doi.org/10.1103/PhysRevB.#1.#3}
  {\emph{Phys.\ Rev.} {\bf B #1} (#2) #3}}
\newcommand\prc[3]{\href{http://dx.doi.org/10.1103/PhysRevC.#1.#3}
  {\emph{Phys.\ Rev.} {\bf C #1} (#2) #3}}
\newcommand\prd[3]{\href{http://dx.doi.org/10.1103/PhysRevD.#1.#3}
  {\emph{Phys.\ Rev.} {\bf D #1} (#2) #3}}
\newcommand\prl[3]{\href{http://dx.doi.org/10.1103/PhysRevLett.#1.#3}
  {\emph{Phys.\ Rev.\ Lett.} {\bf #1} (#2) #3}}
|%%%% Others
\newcommand\econf[3]  {\@spires{ECONF%2C#1%2C#3}
                {{\it eConf\ }{\bf #1} (#2) #3}}
\newcommand\rsi[3]{\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=RSINAK0000#1000001#3000001}
{\emph{Rev.\ Sci.\ Instrum.} {\bf #1} (#2) #3}}
| }}}}}}}}}}}}}}}}}}}}}} "|" is here a comment (catcode defined above) to
| }}}}}}}}}}}}}}}}}}}}}} include parenthesis for emacs to parse properly. 
\newcommand\ibid[3]{{\it ibid.\ }{\bf #1} (#2) #3}
\catcode`\%=14
\catcode`\|=12
% HEPTH's: \hepth{9912999} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hepth}[1]{\href{http://www.arxiv.org/abs/hep-th/#1}{\tt hep-th/#1}}
\newcommand{\hepph}[1]{\href{http://www.arxiv.org/abs/hep-ph/#1}{\tt hep-ph/#1}}
\newcommand{\heplat}[1]{\href{http://www.arxiv.org/abs/hep-lat/#1}{\tt hep-lat/#1}}
\newcommand{\hepex}[1]{\href{http://www.arxiv.org/abs/hep-ex/#1}{\tt hep-ex/#1}}
\newcommand{\nuclth}[1]{\href{http://www.arxiv.org/abs/nucl-th/#1}{\tt nucl-th/#1}}
\newcommand{\nuclex}[1]{\href{http://www.arxiv.org/abs/nucl-ex/#1}{\tt nucl-ex/#1}}
\newcommand{\grqc}[1]{\href{http://www.arxiv.org/abs/gr-qc/#1}{\tt gr-qc/#1}}
\newcommand{\qalg}[1]{\href{http://www.arxiv.org/abs/q-alg/#1}{\tt q-alg/#1}}
\newcommand{\dgga}[1]{\href{http://www.arxiv.org/abs/dg-ga/#1}{\tt dg-ga/#1}}
\newcommand{\accphys}[1]{\href{http://www.arxiv.org/abs/accphys/#1}{\tt accphys/#1}}
\newcommand{\alggeom}[1]{\href{http://www.arxiv.org/abs/alg-geom/#1}{\tt alg-geom/#1}}
\newcommand{\astroph}[1]{\href{http://www.arxiv.org/abs/astro-ph/#1}{\tt astro-ph/#1}}
\newcommand{\chaodyn}[1]{\href{http://www.arxiv.org/abs/chao-dyn/#1}{\tt chao-dyn/#1}}
\newcommand{\condmat}[1]{\href{http://www.arxiv.org/abs/cond-mat/#1}{\tt cond-mat/#1}}
\newcommand{\nlinsys}[1]{\href{http://www.arxiv.org/abs/nlin-sys/#1}{\tt nlin-sys/#1}}
\newcommand{\quantph}[1]{\href{http://www.arxiv.org/abs/quant-ph/#1}{\tt quant-ph/#1}}
\newcommand{\solvint}[1]{\href{http://www.arxiv.org/abs/solv-int/#1}{\tt solv-int/#1}}
\newcommand{\suprcon}[1]{\href{http://www.arxiv.org/abs/supr-con/#1}{\tt supr-con/#1}}
\newcommand{\mathph}[1]{\href{http://www.arxiv.org/abs/math-ph/#1}{\tt math-ph/#1}}
\newcommand{\physics}[1]{\href{http://www.arxiv.org/abs/physics/#1}{\tt physics/#1}}
\newcommand{\Math}[2]{\href{http://www.arxiv.org/abs/math.#1/#2}{\tt math.#1/#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BopHook %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifpdf
\newcommand\Jwatermark[1]{\relax}
\JINST@warnl{ATTENTION!!! watermark disabled. Add it with pdftk 
(use compilaJINSTpdflatex for instance)}
\else
\newcommand\Jwatermark[1]{\special{!userdict begin
/iseven {dup dup 2 idiv 2 mul eq} bind def
/BHend {
  translate rotate
/Courier findfont 30 scalefont setfont
0 0  moveto 0.80 setgray (#1) show grestore}
 bind def
statusdict /duplexmode known
  {statusdict begin duplexmode end}
  {false}
ifelse
  {/bop-hook {gsave iseven {-90 550 570} {+90 50 300} ifelse BHend} def}
  {/bop-hook {gsave         -90 550 570                      BHend} def}
ifelse
end
}\let\JHEP\gobble}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FOOTNOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\skip\footins = 1\bigskipamount plus 2pt minus 4pt

\addtolength{\footnotesep}{1pt}
\renewcommand\footnoterule{%	% NO HYPER...
  \kern-3\p@
  \hrule\@width.4\columnwidth
  \kern2.6\p@}
\newcommand\@makefntext[1]{%
    \parindent 1em%
    \noindent
    \hb@xt@1.8em{\hss\@makefnmark}#1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\contentsname{Contents}
\if@draft\newcommand\listfigurename{List of figures}
	 \newcommand\listtablename{List of tables}\fi
\newcommand\refname{References}
\newcommand\indexname{Index}
\newcommand\figurename{Figure}
\newcommand\tablename{Table}
\newcommand\partname{Part}
\newcommand\appendixname{Appendix}
\newcommand\abstractname{Abstract:}
\newcommand\keywordsname{Keywords:}
\newcommand\receivedname{Received:}
\newcommand\revisedname{Revised:}
\newcommand\acceptedname{Accepted:}
\newcommand\publishedname{Published:}
\newcommand\acknowlname{Acknowledgments}
\newcommand\queriesname{Queries for the author}
\newcommand\today{}
\edef\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}

\setlength\columnsep{20\p@}
\setlength\columnseprule{0\p@}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DEFAULTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pagestyle{JINST}
\pagenumbering{arabic}
\@addtoreset{equation}{section}
\if@preprint
\else
	\let\pagestyle\@gobble
	\let\thispagestyle\@gobble
	\let\pagenumbering\@gobble
\fi
\onecolumn
						
% FOR REQUESTED FRONTMATTER ...
\AtBeginDocument{\bgroup%		SOME NICE (LOCAL) MESSAGES... 
	\def\@APPwarn#1{\JINST@warnl{\protect#1 should appear 
					before \protect\begin{document}}}%
	\def\@APPerr#1{\ClassError{JINST}{\protect#1 should appear 
					before \protect\begin{document}}}%
	\if@author\else\@APPerr{Some \protect\author{...}}\fi
	\if@abstract\else\@APPerr{\abstract{...}}\fi
	\if@preprint
	\else
	        \if@rece\else\@APPerr{\received{...}}\fi
		\if@acce\else\@APPerr{\accepted{...}}\fi
		\if@publi\else\@APPerr{\published{...}}\fi
		\if@keywords\else\@APPwarn{\keywords{...}}\fi
	\fi
	\egroup
	\auto@maketitle}% 
\endinput
%% 
%% End of file `JINST.cls'.

